Topological Planning with Transformers for Vision-and-Language Navigation

Conventional approaches to vision-and-language navigation (VLN) are trained end-to-end but struggle to perform well in freely traversable environments. Inspired by the robotics community, we propose a modular approach to VLN using topological maps. Given a natural language instruction and topological map, our approach leverages attention mechanisms to predict a navigation plan in the map. The plan is then executed with low-level actions (e.g. forward, rotate) using a robust controller. Experiments show that our method outperforms previous end-to-end approaches, generates interpretable navigation plans, and exhibits intelligent behaviors such as backtracking.

==> sections/cvpr_template.tex <==
\section{Introduction}

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the CVPR 2020 web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section,
must be no longer than eight pages in length. The references section
will not be included in the page count, and there is no limit on the
length of the references section. For example, a paper of eight pages
with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for CVPR 2020.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.  

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the \verb'\cvprfinalcopy' command in the document preamble.)  Reviewers:
note that the ruler measurements do not align well with lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $095.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.


\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
techreports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors14} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a techreport for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors14b}''.  Then submit the techreport as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the CVPR70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double blind review policy, you can report results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
   Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.



%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the CVPR 2020 web page for a discussion
of the use of color in your document.

\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: 
\url{https://www.computer.org/about/contact}.

==> sections/intro2.tex <==
\section{Introduction}

Vision-and-language navigation (VLN) is a problem of growing interest which has made significant progress over the last few years. Much of the work has been made using the R2R dataset and the Matterport3DSimulator~\cite{anderson2018vision}, which restricts the agents to jump only to a fixed set of pre-defined locations based on a corresponding set of views. One limitation of this setup is that it is unrealistic and thus an objective of our work is to perform VLN in freely movable spaces.

Due to the nature of the VLN task and setup (discrete position and action), many approaches treat the navigation problem as a sequence prediction or seq2seq~\cite{sutskever2014sequence,anderson2018vision} problem: given a sequence of observations, the agent predicts a sequence of discrete actions. Towards this end, several recent works \cite{tan2019learning,zhu2020vision,ke2019tactical,ma2019regretful,ma2019selfmonitoring,fried_nips2018,wang2019reinforced} utilize single-modal or cross-modal attention on language and vision features combined with unstructured memory (e.g. LSTM~\cite{hochreiter1997long}).

While recurrent models are an effective and common approach to sequential problems, recently the language community has seen breakthroughs in sequence prediction tasks by using attention-based transformer models~\cite{vaswani2017attention} with large amounts of data.% rather than using recurrent models.
These powerful models rely heavily on self-attention mechanisms and have been demonstrated to work tremendously well for language modeling, machine translation, and language generation \cite{devlin2018bert,radford2018improving,radford2019language,brown2020language}, among other tasks. Even for non-sequence prediction tasks, transformers have been effectively used for tasks involving tokenized or discretized inputs, mostly in language but also in vision~\cite{ho2019axial,anonymous2021an}.

Given the discrete, sequential nature of the VLN problem and the importance of single and cross-modal attention for this task as illustrated by prior work, it would be sensible to apply the powerful attention models to the VLN problem. When operating in a free movement environment, rather than directly predicting discrete actions (e.g. forward, rotate left, rotate right) \cite{krantz2020navgraph}, however, an alternative output space for these attention-based models is a series of discrete waypoints in the environment. In particular, the symbolic nature of cognitive-inspired topological maps, which have been explored in the robotics community and have recently gained traction in the vision community \cite{SavinovDosovitskiyKoltun2018_SPTM,Savarese-RSS-19,meng2019scaling,chaplot2020neural}, lends them suitable for the VLN task \cite{thrun1998learning}. Using topological maps promotes efficient planning, interpretable navigation plans, and navigation robustness using cheaper sensors \cite{thrun1998learning,meng2019scaling}.
% Importantly, topological maps are useful for several reasons, including efficiency, interpretability, robustness, and compactness.

Our goal in this work is to unify the powerful attention models, which have been demonstrated to work effectively on tokenized, variable length inputs, with topological maps for the VLN task. By leveraging the self-attention mechanisms inherent in transformers, the agent can attend to both the relevant parts of the language instruction \textit{and} the relevant parts of the navigation environment in order to generate an interpretable plan for where to navigate towards. This planning task shares similarities with language generation and machine translation and therefore can tackled in a similar auto-regressive manner. The resulting agent thus conditions on the current plan generated so far in order to appropriately attend to the relevant parts of the instruction and environment and ultimately compute the next step in the plan. Once this navigation plan has been generated, the agent can execute the plan using a separate, robust low-level controller (which can also be swapped for alternative lower-level controllers which may be desirable for certain situations).

Specifically, we propose a full vision-and-language navigation system which takes the instruction text and image observations as input and produces low-level discrete actions (e.g. turn left, turn right, move forward) as output. The agent is additionally provided with a topological map of the environment which can be manually defined or automatically generated by letting the agent explore the environment beforehand. The agent first goes through a planning phase in which it generates a navigation plan in the topological map as a sequence of nodes. This plan is fixed and does not change throughout the episode. Next, once the plan has been generated, a low-level controller predicts the actions to reach each node (subgoal) until it reaches the final destination.

Given that I have traversed X part of the environment, which parts of the navigation instruction are relevant for computing where to go to next?

The planner is comprised of two main components: a graph neural network (GNN) and a transformer~\cite{vaswani2017attention}. The graph neural network processes the topological map to compute node features which encapsulate the environment structure and connectivity. The node features then get passed along with the navigation instruction to a cross-modal transformer which performs an autoregressive classification on which node to move to next in a manner similar to language translation.

Single-modal attention allows the model to associate related words in a sentence. For example, suppose we have the sentence: ``The bathroom is down the hallway. Walk towards it.'' In this case, the language self-attention can relate the word ``it'' to ``bathroom''. Similarly, during cross-modal attention, the model can relate words like ``bedroom'' to the corresponding place in the indoor environment. Moreover, during planning, it is important to attend to the words at the right time. For example, at the beginning of the trajectory the first few instruction steps may be more relevant than the last few instruction steps.

Additionally, transformers are naturally suitable for this task not only because they facilitate single and cross modal attention, but also because they are permutation invariant with respect to the input. Unlike a recurrent model such as an LSTM~\cite{hochreiter1997long}, the ordering of the input (ie. topological graph nodes) does not affect the output of the transformer (unless some form of positional encoding used).

% In summary, our contributions are the following:
% \begin{itemize}
%     \item asdf
%     \item asdf
%     \item asdf
% \end{itemize}

% This separation between planning and control allows interpretable plans and robust, swappable controllers.
% Moreover, it is natural to solve the navigation planning problem using an autoregressive approach, similar to machine translation and language generation.
% A separate observation about recent VLN models is that they largely operate as black-box models

% The VLN setup in Room2Room (R2R)~\cite{anderson2018vision} makes it natural for these approaches (e.g. \cite{anderson2018vision}) to treat the navigation problem as sequence prediction or seq2seq~\cite{sutskever2014sequence} problems. Concurrently, the language community has seen a revolution in

==> sections/method_backup.tex <==
Before planning could take place, the agent must first construct a robust topological representation of the environment. Specifically for this problem, good topological maps should: 1) cover a large proportion of traversable area, such that there always exists a node close enough to the any start and goal position; 2) contain rich information in nodes and edges to enable autoregressive planning from this topological representation only; and 3) consists of connected nodes that are reachable to a high probability when executing the plan in simulation.

In our setup, the agent first explores by traversing between randomly sampled waypoints in the simulated environment. Then exploration trajectories are sparsified by a reachability estimator as proposed by [todo cite meng] to form a graph, and we repeat the process multiple times for each environment and merge the resultant graphs for robustness. To study the efficacy of agent-generate maps, we process pre-defined topological graphs from the R2R [todo cite] dataset in a similar fashion and conduct experiments.

For constructing the topological graphs, we assume the agent has odometry sensor providing its coordinates and orientation such that the relative translation from node to node is known. Note that this does not need to be calibrated to the environment's coordinates, but only need to be consistent throughout the exploration trajectory. We use this information to categorize each edge by its approximate orientation and length. Each node is represented by an RGBD panoramic observation at its corresponding position rotated to a consistent orientation.

==> sections/notes.tex <==
\section{Notes}

Story 1
\begin{itemize}
    \item VLN is a problem of growing interest. Many approaches use attention on language + vision features with unstructured memory (e.g. LSTM).
    \item NLP community has seen significant advances in language modeling and translation with the advent of transformers, which essentially perform attention on crack. They have been shown to work really well for sequence prediction and even discretized prediction (e.g. image patches).
    \item Separately, the visual navigation community has also moved towards structured memory and discretized representations of indoor spaces through topological maps, which have been around in the robotics community for a long time and connect more easily with language than metric maps. Topological maps allow for efficient planning, interpretable plans, robustness to cheap cameras/sensors.
    
\end{itemize}

\begin{itemize}
    \item Leverage topo maps used by robotics community
    \item Leverage powerful attention mechanisms and sequential prediction models from NLP community
\end{itemize}

Vision-and-language navigation (VLN) has made a lot of progress over the last few years.

Much of the work is based on navigating in a simplified navigation graph setting and using recurrent, cross-modal sequence-to-sequence models to map from observation and instruction to action direction. However, most works don't utilize maps, which have proven to be extremely useful by the robotics community. The implication is that the latent memory of the recurrent models can capture the necessary and relevant information

In particular, topological maps have a natural synergy with natural language due to the discrete and symbolic nature of both modalities.

Our goal is to perform VLN using topological maps by leveraging the powerful attention mechanisms and sequence prediction models that have been demonstrated to work well in the natural language community. Our key observation is that path planning in a topological map draws many similarities to language modeling and machine translation -- both problems can be approached as autoregressive sequence prediction.

In particular, we hypothesize that powerful attention mechanisms are essential for learning to follow and execute natural language navigation instructions. Different parts of the instruction may refer to different parts of the environment. For example, asdf.

Transformers are also a naturally suitable approach because it is invariant to node ordering.

Insights from working on this:
\begin{itemize}
    \item Topo map representation has a BIG impact. Verify this experimentally
\end{itemize}

What are some useful properties of topological maps?

\begin{itemize}
    \item Unique / able to localize properly
    \item Some level of geometric information to resolve ambiguities
    \item I would argue that it should not be orientation dependent
\end{itemize}

Challenges:
\begin{itemize}
    \item Orientation of topo map node
    \item Density of nodes
    \item Reachability between nodes
    \item Making sure that start/goal are close to some topo node by some measure
    \item Moving to regions that weren't traversed during exploration
\end{itemize}

Effects of different topo map representations:
\begin{itemize}
    \item If you only drop nodes along exploration trajectory, you cannot move outside of that region at test time. For example, you'll never go to the other side of the table.
    \item How to navigate to precise goal position
    \item How densely placed should nodes be? Use of metric maps?
    \item How does performance change on different topo map representations when we feed in no instruction?
    \item How does performance change when using single exploration maps vs. merged multiple exploration maps? This effect is more drastic for single-room envs.
\end{itemize}

From Improving using image-text pairs: In this setting, a high-probability path is typically generated by performing beam search through the environment and ranking paths according to either: (1) their probability under a ‘follower’model [Chasing Ghosts 3, Speaker-follower 8, Tactical rewind: 13, Self-monitoring: 20, The regretful agent 21, reinforced cross-modal matching and self-supervised imitationlearning for vision-language navigation 30, Look before you leap 31], as in Figure 1 (left), or (2) by how well they explain the instruction according to a ‘speaker’ (instruction generation) model [Speaker-follower 8, Learning to navigate unseen environments with backtranslation/environmental dropout 28],as in Figure 1 (center). In contrast, we use beam search with an existing agent model [28] to generate a set of candidate paths, which we then evaluate usingour discriminative path-instruction compatibility model, as in Figure 1 (right).

Related works:
\begin{itemize}
    \item bringmeaspoon
    \item Speaker Follower
    \item Are You Looking? Grounding to Multiple Modalities in Vision-and-Language Navigation
    \item Tactical Rewind: Self-Correction via Backtracking in Vision-and-Language Navigation
    \item The Regretful Agent: Heuristic-Aided Navigation through Progress Estimation
    \item Self-Monitoring Navigation Agent via Auxiliary Progress Estimation
    \item Chasing Ghosts: Instruction Following as Bayesian State Tracking
    \item Reinforced Cross-Modal Matching and Self-Supervised Imitation Learning for Vision-Language Navigation
    \item Learning to Navigate Unseen Environments: Back Translation with Environmental Dropout
    \item Vision-Language Navigation with Self-Supervised Auxiliary Reasoning Tasks
    \item VLN-CE
    \item Improving Vision-and-Language Navigation with Image-Text Pairs from the Web
\end{itemize}

==> sections/related_work_old.tex <==
\section{Related Work}

\begin{figure}
     \centering
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figs/internal-deadline-figs/topo-map-r2r.png}
         \caption{Topological map. White represents traversable regions.}
         \label{fig:topological-map-topomap}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figs/internal-deadline-figs/exploration-trajectory.png}
         \caption{Exploration trajectory.}
         \label{fig:topological-map-explore-traj}
     \end{subfigure}
    \caption{Topological map and explore trajectory.}
    \label{fig:topological-map}
\end{figure}

\begin{figure}
\begin{center}
  \includegraphics[width=0.8\linewidth]{figs/internal-deadline-figs/Polar-Coord.pdf}
\end{center}
  \caption{Directed edge labels for the topological map are represented as discretized polar coordinates.}
\label{fig:polar-coord}
\end{figure}

\subsection{Vision-and-Language Navigation}

% From Majumdar et al.: Path Selection in VLN.In VLN [4], an agent is required to follow a nav-igation instruction from a start location to a goal. While most existing worksfocus on the setting in which the test environments are previously unseen, manyalso consider the scenario in which the test environment is previously exploredand stored in memory (i.e., fully observable). In this setting, a high-probabilitypath is typically generated by performing beam search through the environmentand ranking paths according to either: (1) their probability under a ‘follower’model [3,8,13,20,21,30,31], as in Figure 1 (left), or (2) by how well they explainthe instruction according to a ‘speaker’ (instruction generation) model [8, 28],as in Figure 1 (center). In contrast, we use beam search with an existing agentmodel [28] to generate a set of candidate paths, which we then evaluate usingour discriminative path-instruction compatibility model, as in Figure 1 (right).

% The seminal work of Anderson et al.~\cite{anderson2018vision} introduced the problem of vision-and-language navigation (VLN) using Room-to-Room (R2R) dataset along with the Matterport3D Simulator. Since then, significant progress in VLN has been made. Most works focus on navigation in previously unseen environments, but some

Our problem setup is related to approaches which assume the test environment has been previously explored \cite{anderson2019chasing,fried_nips2018,ke2019tactical,ma2019selfmonitoring,ma2019regretful,tan2019learning,wang2018look,wang2019reinforced}. These approaches use the Matterport3D Simulator~\cite{anderson2018vision}, usually assuming a panoramic action space ~\cite{fried_nips2018} and allowing the agent to teleport to and from a fixed set of pre-defined locations in the environment. This setup promotes fast iteration and evaluation of different VLN approaches, but ignores (1) the problem of associating action directions with nodes in the graph, and (2) the motion and feasibility problem of moving from one location to another. In contrast, in our work the agent builds a topological map of the environment from ground up in an online fashion when provided with specific exploration trajectories, and uses the local controller to convert from a predicted path in the topological map to low-level discrete actions.

Three particularly related works: EGP, VLN-BERT, VLNCE.
% In such approaches, candidate paths are generated and ranked using a follower or speaker model \cite{majumdar2020vlnbert}.

% Moreover, asdf use a path ranking approach based on candidate route generation using a follower model~\cite{fried_nips2018}. Our approach is orthogonal in that the follower model can be replaced with our model and then used in conjunction with many of these approaches.

Deng et al.~\cite{deng2020evolving} also operates under a similar setting, using the pre-defined navigation graph to teleport from one location to another. Their approach is related to ours because they perform planning in a global graph but they have a fundamentally different assumption that the environment has not been previously seen before. Thus, the agent can explore the environment at test-time and take multiple actions to correct for mistakes, such as when the agent goes to the wrong location. In other words, the agent can take multiple attempts to execute the instruction. In contrast, our setup assumes prior exploration of the environment. Therefore, it is desirable to plan only a single time rather than multiple times.
% They also do this weird thing where they can see the observations of all possible actions (1-step lookahead).
% is more like a one-shot prediction where we take into account the global understanding of the environment and then determine where to go.

A few differences with EGP:
\begin{itemize}
    \item They focus on VLN in un-seen environments. Thus, the agent is able to go to many different parts of the environment until it finally reaches the goal. Although they do not propose a mapping approach (rather, they assume the map is pre-defined), their approach is designed under the assumption of gradually building a ``map'' as the agent traverses the environment. Thus, they keep track of unvisited ``leaf'' nodes and can consistently choose new unvisited leaf nodes as they explore the environment. This allows them to correct for mistakes, such as when the agent goes in the wrong direction. In contrast, our is more like a one-shot prediction where we take into account the global understanding of the environment and then determine where to go.
    \item The closest analogy we can make is a similar model which predicts the navigation destination in one shot. However, this isn't a fair comparison for them because their approach is designed assuming map information isn't available at the beginning.
    \item The navigation graph in their work is the same as the Matterport graph. They don't provide a solution for how to actually build this graph.
\end{itemize}
% From fried: using a panoramic action space with panoramic representation, convertedwith built-in mapping from low-level visuomotor control
% erceives a360-degree panoramic view of its surrounding scene from its current location, which is discretizedinto 36 view angles (12 headings×3 elevations with 30 degree intervals – in our implementation).Each view angleiis represented by an encoding vectorvi. At each location, the agent can only movetowards a few navigable directions (provided by the navigation environment) as other directions canbe physically obstructed (e.g. blocked by a table). Here, in our action space the agent only needs tomake high-level decisions as to which navigable direction to go to next, with each navigable directionjrepresented by an encoding vectoruj.
% navigable direction are obtained by concatenating an appearance feature (ConvNet feature extractedfrom the local image patch around that view angle or direction) and a 4-dimensional orientationfeature[sinψ; cosψ; sinθ; cosθ], whereψandθare the heading and elevation angles respectively.Also, we introduce aSTOPaction encoded byu0=−→0. The agent can take thisSTOPaction when itdecides it has reached the goal location (to end the episode).
% The agent then chooses a navigable directionuj(with probabilitypj) to go to the adjacent locationalong that direction (oru0to stop and end the episode). We use a built-in mapping that seamlesslytranslates our panoramic perception and action into visuomotor control such as turning and moving.

Attention in visual navigation (scene memory transformer, image-text pairs, Towards Learning a Generic Agent forVision-and-Language Navigation via Pre-training)

\subsection{Topological Maps and Structured Memory for Visual Navigation}

Early learning-based approaches to visual navigation were reactive \cite{zhu2017target,dosovitskiy2016learning} or based on unstructured memory \cite{mnih2016asynchronous,mirowski2016learning}. Several works investigate using explicit representation of environments, such as metric map-based representations \cite{parisotto2018neural,gupta2017cognitive,gupta2017unifying,gupta2019cognitive,zhang2017neural,chaplot2019learning}. \cite{fang2019scene} propose storing observations and poses. Alternative representations inspired by cognitive science and the robotics community propose learning-based visual navigation using topological maps \cite{SavinovDosovitskiyKoltun2018_SPTM,chaplot2020neural,Savarese-RSS-19,meng2019scaling}. \cite{anderson2019chasing} uses metric map for VLN (right?) with mediocre performance results.

\subsection{Robotics Style}

Language and navigation, topological maps for navigation.

\subsection{Language Generation and Translation}

\begin{itemize}
    \item Attention is All You Need
    \item BERT
    \item ViLBERT
    \item VL-BERT
    \item GPT, GPT-2, GPT-3
    \item ...
\end{itemize}
